Capturing Conditional Dependence via Auto-regressive Diffusion Models

Diffusion models have demonstrated appealing performance in both image and video generation. However, many works discover that they struggle to capture important, high-level relationships that are present in the real world. For example, they fail to learn physical laws from data, and even fail to understand that the objects in the world exist in a stable fashion. This is due to the fact that important conditional dependence structures are not adequately captured in the vanilla diffusion models. In this work, we initiate an in-depth study on strengthening the diffusion model to capture the conditional dependence structures in the data. In particular, we examine the efficacy of the auto-regressive (AR) diffusion models for such purpose and develop the first theoretical results on the sampling error of AR diffusion models under (possibly) the mildest data assumption. Our theoretical findings indicate that, compared with typical diffusion models, the AR variant produces samples with a reduced gap in approximating the data conditional distribution. On the other hand, the overall inference time of the AR-diffusion models is only moderately larger than that for the vanilla diffusion models, making them still practical for large scale applications. We also provide empirical results showing that when there is clear conditional dependence structure in the data, the AR diffusion models captures such structure, whereas vanilla DDPM fails to do so. On the other hand, when there is no obvious conditional dependence across patches of the data, AR diffusion does not outperform DDPM.

==> 0_config/init_load.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input

%-----------------------------------
\pdfoutput=1

\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm,amsfonts}
\usepackage{array}
\usepackage{authblk}
\usepackage{babel}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{colortbl}% http://ctan.org/pkg/xcolor
\usepackage{enumitem}
\usepackage[T1]{fontenc}    
\usepackage{framed}
\usepackage{graphicx}
\usepackage[colorlinks, linkcolor=red, anchorcolor=blue, citecolor=blue]{hyperref}
\usepackage{indentfirst}
\usepackage[utf8]{inputenc}
\usepackage{lipsum}        
\usepackage{makecell}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{xparse}
% \usepackage{subcaption}
\usepackage[framemethod=default]{mdframed}
\usepackage{microtype}     
\usepackage{multicol}
\usepackage{multirow}
\usepackage[numbers]{natbib}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{tablefootnote}
\usepackage{url}            % simple URL typesetting
\usepackage{wrapfig,lipsum}
\usepackage{xcolor}         % colors
\usepackage{xspace}

\usepackage{subfigure}
\usepackage[capitalize,noabbrev]{cleveref}


\usepackage{doi}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
% \renewcommand{\baselinestretch}{1.1}
\parindent 15pt

\usepackage{lmodern}


% For paper revision:
\newcommand{\xh}[1]{\textcolor[HTML]{66CCFF}{#1}}
\def \dz {\textcolor{red}}

==> 0_config/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures

\newcommand{\figleft}{{\em (Left)}}

\newcommand{\name}{{{RDS}}}


\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\hanze}[1]{{\textcolor{orange}{#1} }}

\newcommand{\issue}[1]{{\textcolor{purple}{#1} }}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~(\ref{#1})}
% Reference to an equation, upper case
%\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}

\def\cN{{\mathcal{N}}}
% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvzeta{{\mathbf{\zeta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\cR{{\mathcal{R}}}
\def\EE{{\mathbb{E}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vrho{{\bm{\rho}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

%

\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny{#1}};}}
% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}[2]{\mathrm{KL}\left(#1 \big\| #2\right)}
\newcommand{\FI}[2]{\mathrm{FI}\left(#1 \big\| #2\right)}
\newcommand{\TVD}[2]{\mathrm{TV}\left(#1, #2\right)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\newcommand{\der}{\mathrm{d}}
\newcommand{\fder}{\mathrm{D}}
\newcommand{\rgrad}{\mathrm{grad}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Table settings

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


\newcommand{\rbkwx}{\rvx^{\gets}}
\newcommand{\bkwx}{\vx^{\gets}}
\newcommand{\rbkwv}{\rvv^{\gets}}
\newcommand{\bkwp}{p^{\gets}}
\newcommand{\ourmethod}{\text{RS-DMC}}



==> 0_contents/040AnalysisARD.tex <==
\section{Theoretical Guarantees for AR Diffusion}

% In this section, we will first provide the main theorem on the convergence of AR diffusion inference and compare it with that in typical diffusion.
% Then, we explain that the AR diffusion model may have better performance because the gap between the conditional distributions of generated and ground truth data will blow up in typical DDPM when some tokens are drawn from a low-density area. \dz{this is confusing, tokens drawn from a low-density area? this looks like you are doing finite-sample training ..}
% After that, we will provide the proof sketch and core lemmas.

In this section we provide the theoretical analyses of the AR diffusion models.
We first analyze the efficacy of AR diffusion in capturing the conditional dependence structures in the data, and compare against the vanilla diffusion models.
We then analyze in general the inference and training performance of AR diffusion.
We demonstrate that, compared with typical DDPM, its gradient complexity increases by a factor of $K$ (the number of data patches) during the inference time, but it is practical for large-scale applications.

\subsection{AR diffusion captures conditional dependence}
% Besides, the gap between the conditional distributions of generated and ground truth data is given as follows.
We first provide a lemma on the convergence of the AR diffusion-generated conditional distributions towards the ground truth data distribution.
We then provide another lemma to contrast it against the distributions generated by vanilla diffusion models.
\begin{lemma}
    \label{lem:condi_rtk_error_eachk_main}
    For any $k\ge 1$, for any $k$-tuples $\vx_{[1:k]}\in\R^{d_1+d_2+\ldots+d_k}$, we consider the SDE.~\ref{sde:prac_condi_reverse} to simulate the reverse process of SDE.~\ref{sde:ideal_condi_forward}, with a proper design of the time sequence $\{t_r\}_{r=0}^R$,
    we have
    \begin{equation*}
        \begin{aligned}
            & \KL{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}{\hat{p}_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}\\
            & \lesssim e^{-2T}\cdot \left(2Ld_{k+1} + \E_{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}\left[\|\rvy\|^2\right] \right)\\
            & \quad + \eta\cdot \sum_{r=0}^{R-1} \tilde{L}_{k+1,r}(\vtheta|\vx_{[1:k]}) +  d_{k+1}L^2R\eta^2\\
            &\quad + d_{k+1}T\eta+ \eta \E_{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}\left[\|\rvy\|^2\right].
        \end{aligned}
    \end{equation*}
\end{lemma}
The above means that given the data patch $\vx_{[1:k]}$ that is being conditioned upon, we can always choose a small enough step size $\eta$ and a large enough convergence time $T$, so that the conditional distribution converges to any desired accuracy $\epsilon$: $\KL{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}{\hat{p}_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})} \leq \epsilon$.

% \textcolor{red}{Put Lemma B.2 in the other file here to be the main result.
% Assume that $p(\mathbf{x}_{[1:k]})$ is $\sigma$-subGaussian. 
% Then we should get that $\E_{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}\left[\|\rvy\|^2\right]$ in that upper bound scales as $\sigma^2$.
% On the other hand, the error in the conditional KL, achieved by the vanilla diffusion model would scales as $e^{\sigma^2} \sigma^d$.}


% \dz{we need a paragraph or subsection to give a complete and precise comparison with the diffusion model, i.e., the case of K=1}.

On the other hand, if one only performs score matching over the joint distributions $q_{T-t}(\vx_{[1:K]})$, the convergence of the diffusion model is in terms of $\KL{p_*(\vx_{[1:K]})}{\hat{p}_*(\vx_{[1:K]})}$.
In the Lemma below, we demonstrate that even for the Gaussian target, and even if the KL divergence between the joint distributions are arbitrarily small, the KL divergence between the conditional distributions can remain arbitrarily large.
\begin{lemma}
\label{lem:lower_bound}
Consider random vectors $\rvy\in\mathbb{R}^{d_{k+1}}$ and $\vx\in\mathbb{R}^{d_1+d_2+\dots+d_k}$.
For any error threshold $\varepsilon\in(0,1/2]$ and for any $M\in\mathbb{R}$, there exists a pair of Gaussian probability densities $\left( p_*(\rvy,\vx), \hat{p}_*(\rvy,\vx) \right)$, such that 
$\KL{p_*(\rvy,\vx)}{\hat{p}_*(\rvy,\vx)} \leq \varepsilon$, while $\KL{p_*(\rvy|\vx)}{\hat{p}_*(\rvy|\vx)} > M^2 \cdot \|\vx_{(1:d_{k+1})}\|^2$.
\end{lemma}

\subsection{Inference performances of AR diffusion}
Building upon Lemma~\ref{lem:condi_rtk_error_eachk_main}, we deliver the theoretical result on the sampling error of AR diffusion model on the joint distributions over all the random variables $\vx_{[1:K]}$.
\begin{theorem}
    \label{thm:main_}
    Suppose Assumption~\ref{a2}-\ref{a3} hold, 
    \begin{equation*}
        \delta\le \Big(0, \ln \sqrt{(4L)^{-2}+1}+(4L)^{-1}\Big]
    \end{equation*}
    if Alg.~\ref{alg:ard_outer} chooses the time sequence $\{\eta_r\}_{r=0}^{R-1}$ as
    \begin{equation*}
        \eta_r = \left\{
            \begin{aligned}
                & \eta && \text{when}\quad 0\le r<M\\
                & \eta/(1+\eta)^{r-M+1} && \text{when}\quad M\le r<N\\
                & \eta && \text{when}\quad N\le r\le R
            \end{aligned}
        \right.
    \end{equation*}
    where 
    \begin{equation*}
        M=\frac{T-1}{\eta},\quad N=M+\frac{2\ln(1/\delta)}{\eta},\quad \text{and}\quad R=N+\frac{\delta}{\eta},
    \end{equation*}
    then, the generated samples
    $[\hat{\rvx}_1, \hat{\rvx}_2, \ldots, \hat{\rvx}_K]$ follows the distribution $\hat{p}_*$, which satisfies
    \begin{equation*}
         \begin{aligned}
             &\KL{p_*}{\hat{p}_*}\lesssim  2e^{-2T}L\cdot \left(m_0+ d\right)\\
            &\quad+ (L^2R\eta^2+T\eta)\cdot d  + \eta m_0 + \eta KR\cdot \epsilon_{\mathrm{score}}^2.
         \end{aligned}
    \end{equation*}
\end{theorem}
\begin{remark}
% \dz{we may mention why to consider such a special time sequences? any intuition?}
    To achieve the KL convergence, e.g., $\KL{p_*}{\hat{p}_*}\le \epsilon^2$ for the generated data, we only require the hyper-parameters to satisfy $T = \tilde{\Theta}(1)$,
    \begin{equation*}
        \eta = \tilde{\Theta}(L^{-2}d^{-1}\epsilon^{-2})\quad \text{and}\quad \epsilon_{\mathrm{score}}=\tilde{O}(K^{-1/2}\epsilon).
    \end{equation*}
    Under these conditions, the total gradient complexity of the inference process will be at an $\tilde{O}(KL^2d\epsilon^{-2})$ level.
    Compared with typical DDPM (corresponding to the special case $K=1$ in our setting), this complexity will have an additional factor of $K$, which means AR diffusion usually requires more inference steps to achieve the same generation quality and matches people's general perception in empirical studies.
    From the training perspective, the average dimension of the estimated score in AR diffusion is only $1/K$ of that in typical diffusion.
\end{remark}

\paragraph{Proof sketch of Theorem~\ref{thm:main_}.}
To obtain Theorem~\ref{thm:main_}, we start by checking the gap between the distribution of generated $\hat{p}_*$ and ground-truth data distribution $p_*$, which is written as
\begin{equation}
    \small
    \label{ineq:kl_gap_accu}
    \begin{aligned}
        \KL{p_*}{\hat{p}_*}\le \KL{p_{*,1}}{\hat{p}_{*,1}} + \sum_{k=1}^{K-1} \E_{\rvx_{[1:k]}\sim p_{*,[1:k]}}\\
        \left[\KL{p_{*,k+1|[1:k]}(\cdot|\rvx_{[1:k]})}{\hat{p}_{*,k+1|[1:k]}(\cdot|\rvx_{[1:k]})}\right]
    \end{aligned}
\end{equation}
following from the chain rule of $f$ divergence.
In Alg.~\ref{alg:ard_inner}, for any given $\vx_{[1:k]}$, $\hat{p}_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})$ and $p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})$ are the target and output distributions, which is presented as $q^\gets_T$ and $\hat{q}_T$, respectively. 
Moreover, their KL divergence satisfies
\begin{equation*}
    \begin{aligned}
        &\KL{q^\gets_T}{\hat{q}_T}\le \KL{{q}^\gets_0}{\hat{q}_0}\\
        &\qquad + \underbrace{ \sum_{r=0}^{R-1} \E_{{\rvy}^\gets\sim {q}^\gets_{t_r}}\left[\KL{{q}^\gets_{t_{r+1}|t_r}(\cdot|{\rvy}^\gets)}{\hat{q}_{t_{r+1}|t_r}(\cdot|{\rvy}^\gets)}\right]}_{\text{reverse transition error}}.
    \end{aligned}
\end{equation*}
Considering that both $\{{q}^\gets_t\}_{t=0}^T$ and $\{\hat{q}_t\}_{t=0}^T$ are simulating reverse OU processes, the initialization error, i.e., $\KL{{q}^\gets_0}{\hat{q}_0}$, can be adaptively controlled by
\begin{equation}
    \label{ineq:init_error_main}
    \begin{aligned}
        &\KL{{q}^\gets_0(\cdot|\vx_{[1:k]})}{\hat{q}_0(\cdot|\vx_{[1:k]})}\\
        &\le e^{-2T}\cdot \left(2Ld_{k+1} + \E_{p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})}\left[\|\rvy\|^2\right] \right)
    \end{aligned}
\end{equation}
following the convergence of the standard OU process.
Although the upper bound of initialization error in our settings contains the unbounded variables, i.e., $\vx_{[1:k]}$ rather than a uniform bound in typical DDPM analyses.
For the reverse transition error, the Girsanove Theorem allows us to decompose it to the sum of score estimation error, i.e.,
\begin{equation*}
    \small
    \begin{aligned}
        \sum_{r=0}^{R-1} \eta_r\cdot \E_{\tilde{\rvy}_{t_r}}\left[\left\|\vs_{\vtheta}(\tilde{\rvy}_{t_r}|T - t_r,\vz )-  \grad\ln q_{T-t_r}(\tilde{\rvy}_{t_r})\right\|^2\right]
    \end{aligned}
\end{equation*}
and the discretization error, i.e.,
\begin{equation*}
    \small
    \begin{aligned}
        \sum_{r=0}^{R-1} \E_{\tilde{\rvy}_{[0:T]}}\left[\int_{t_r}^{t_{r+1}} \left\|\grad\ln q_{T-t_r}(\tilde{\rvy}_{t_r})-  \grad\ln q_{T-t}(\tilde{\rvy}_t) \right\|^2 \der t \right].
    \end{aligned}
\end{equation*}
Suppose there is an upper bound $\eta$ for all of the dynamics step size $\eta_r$, then the score estimation error will be coincidentally controlled by a partial sum of the score training error provided in Assumption~\ref{a3}, i.e.,
\begin{equation*}
     \eta\cdot  \sum_{r=0}^{R-1} \tilde{L}_{k+1,r}(\vtheta|\vx_{[1:k]}).
\end{equation*}
For the discretization error, we divide the entire reverse process into two segments, i.e., $[0, T-\delta]$ and $(T-\delta, T]$. 
For the first segment, we check the dynamics of 
\begin{equation*}
    E_{s,t}:=\E_{\tilde{\rvy}_{[0:T]}\sim \tilde{Q}_{[0:T]}}\left[\left\|\grad\ln \tilde{q}_{t}(\tilde{\rvy}_{t})-  \grad\ln \tilde{q}_{s}(\tilde{\rvy}_s) \right\|^2 \right]
\end{equation*}
with It\^o calculus and bound the differential inequality coefficients with a similar approach to~\cite{benton2024nearly}. 
For the second segment, we choose a sufficient small  $\delta$ to satisfy the condition of Lemma \ref{lemma:c.9}, then the Lipschitz property of the score function $\grad \ln q_t$ ($t\in[0,\delta]$) can be guaranteed, thereby allowing the discretization error to be bounded by the difference between particles.
Under these conditions, Lemma~\ref{lem:condi_rtk_error_eachk_main} can summarize an adaptive convergence.
Although the adaptive convergence of Alg.~\ref{alg:ard_inner} contains the unbounded $\vx_{[1:k]}$, taking the expectation on $\vx_{[1:k]}$ will make the conditional second moment and the partial sum of the score training error have uniform upper bounds following from Lemma~\ref{lem:init_second_moment_bounded_main} and Assumption~\ref{a3}, respectively.
Under these conditions, the KL divergence accumulates linearly across the patches following Eq.~\ref{ineq:kl_gap_accu}
Theorem~\ref{thm:main_} is thus proved.  




==> 0_contents/050Experiments.tex <==
\section{Experiment}
\label{sec:exp}
In this section, we demonstrate the advantages of AR Diffusion over DDPM and the tightness of the sampling performance bound of AR Diffusion provided in Theorem~\ref{thm:main_} in two synthetic experiments, where the image data contains feature dependencies.
\begin{figure}[]
\centering
    \hfill
    \subfigure[Task 1]{\label{fig:task1}\includegraphics[width=0.2\textwidth]{figures/task1_v2.pdf}}
    \hfill
    \subfigure[Task 2]{\label{fig:task2}\includegraphics[width=0.2\textwidth]{figures/task2_v2.pdf}}
    \hfill
\vspace{-0.1in}
\caption{Visualization of Task 1 and Task 2. In Task 1, a patch size of 16 ensures that correlated features (sun and shadow) are located in different patches. In contrast, Task 2 uses a patch size of 8, which disrupts the dependency between the square's lengths by segmenting them into different patches.}
\vspace{-0.15in}
\label{fig:task_vis}
\end{figure}


\paragraph{Synthetic Tasks.}Specifically, following the setting \cite{han2025can}, we consider the following synthetic tasks in \cref{fig:task_vis}: (1) Task 1: Contains three elements representing the sun, the flagpole, and the shadow, where geometric features such as the height of the sun and the length of the shadow are correlated and satisfy the constraint \( \frac{l_1}{h_1} = \frac{l_2}{h_2} \); (2) Task 2: Contains two squares, where the side length \( l_1 \) of the square in the upper part and the side length \( l_2 \) of the square in the lower part satisfy the constraint \( l_2 = 1.5l_1 \). Task 1 is an abstraction of common light and shadow phenomena in the real world. In this setting, the length of an object's shadow is determined by multiple factors, such as the height of the sun and the height of the object. Task 2, on the other hand, attempts to minic certain physical rules, such as perspective effects, where objects appear larger when they are closer to the lower observation point.

\begin{figure*}[]
\centering
    \hfill
    \subfigure[Training Data]{\label{fig:task1_tr}\includegraphics[width=0.24\textwidth]{figures/task1_tr.pdf}}
    \hfill
    \subfigure[Inference: AR Diffusion]{\label{fig:task1_ar}\includegraphics[width=0.24\textwidth]{figures/task1_ar.pdf}}
    \hfill
    \subfigure[Inference: DDPM]{\label{fig:task1_ddpm}\includegraphics[width=0.24\textwidth]{figures/task1_ddpm.pdf}}
    \hfill
    \subfigure[Training: Diffusion Loss]{\label{fig:task1_loss}\includegraphics[width=0.22\textwidth]{figures/task1_loss_distribution.pdf}}
    \hfill
\vspace{-0.15in}
\caption{\textbf{Comparison of AR Diffusion and DDPM Performance on Task 1.} \Cref{fig:task1_tr} demonstrates the validity of the evaluation method using the training data as a baseline.  \Cref{fig:task1_ar} and \Cref{fig:task1_ddpm} illustrate the performance of AR Diffusion and DDPM during the inference phase, showing that AR Diffusion better captures inter-feature dependencies with a higher \( R^2 \). \Cref{fig:task1_loss} presents the difference in training loss between DDPM and AR Diffusion, denoted as \( \delta \). For most training steps, AR Diffusion's training loss is lower than that of DDPM, with \( \delta > 0 \).}
\vspace{-0.15in}
\label{fig:task_1_dis}
\end{figure*}



% \begin{figure*}[]
% \centering
%     \hfill
%     \subfigure[Training Data]{\label{fig:eo_tr}\includegraphics[width=0.23\textwidth]{figures/eo_even_0000.png}}
%     \hfill
%     \subfigure[Inference Phase]{\label{fig:eo_ar_ddpm_infer}\includegraphics[width=0.26\textwidth]{figures/mnist-eo-unet.pdf}}
%     \hfill
%     \subfigure[Training Phase]{\label{fig:eo_ar_ddpm_loss}\includegraphics[width=0.24\textwidth]{figures/mnist-eo_loss_distribution_unet.pdf}}
%     \hfill
% \vspace{-0.15in}
% \caption{\textbf{Comparison of AR Diffusion and DDPM Performance on Odd and Even Setting.} \Cref{fig:eo_tr} shows the odd-even setting based on MNIST, where each training sample contains four sub-images with consistent parity. \Cref{fig:eo_ar_ddpm_infer} calculates the generated samples that satisfy the predefined dependencies, and AR Diffusion significantly outperforms DDPM. The dashed line represents the application of the testing method to the training data. We observe that nearly 100\% of the training data satisfies the predefined inter-feature dependencies. \Cref{fig:eo_ar_ddpm_loss} shows the training loss of AR Diffusion and DDPM, where DDPM's training loss is higher than AR Diffusion's for nearly 70\% of the training steps.}
% \vspace{-0.15in}
% \label{fig:eo_ar_ddpm_unet}
% \end{figure*}


% \begin{figure*}[]
% \centering
%     \hfill
%     \subfigure[Training Data]{\label{fig:seq_tr}\includegraphics[width=0.23\textwidth]{figures/seq_0-3_0009.png}}
%     \hfill
%     \subfigure[Inference Phase]{\label{fig:seq_ar_ddpm_infer}\includegraphics[width=0.26\textwidth]{figures/mnist-seq-unet.pdf}}
%     \hfill
%     \subfigure[Training Phase]{\label{fig:seq_ar_ddpm_loss}\includegraphics[width=0.24\textwidth]{figures/mnist-seq_loss_distribution_unet.pdf}}
%     \hfill
% \vspace{-0.15in}
% \caption{\textbf{Comparison of AR Diffusion and DDPM Performance on Arithmetic Sequence Setting.}\Cref{fig:seq_tr} shows the arithmetic sequence setting based on MNIST, where each training sample contains four sub-images that satisfy the arithmetic sequence. \Cref{fig:seq_ar_ddpm_infer} shows that over 80\% of the samples generated by AR Diffusion satisfy the predefined dependencies, while DDPM only has less than 50\% of its generated samples meeting the dependencies.  The dashed line represents the application of the testing method to the training data. We observe that nearly 100\% of the training data satisfies the predefined inter-feature dependencies. \Cref{fig:seq_ar_ddpm_loss} shows the training loss of AR Diffusion and DDPM, where for 60\% of the training steps, DDPM's training loss is higher than that of AR Diffusion.}
% \vspace{-0.15in}
% \label{fig:seq_ar_ddpm_unet}
% \end{figure*}


\paragraph{Setup and Evaluation.} 
Based on the designed Task 1 and Task 2, we train AR Diffusion and DDPM from scratch while ensuring that these two models have comparable parameters. Moreover, due to the synthetic data containing only sufficiently simple elements, we can directly extract relevant geometric features from the generated images, as the evaluation method proposed in previous work \cite{han2025can}. After extracting these features, we can further examine whether the generated images satisfy the predefined rules to evaluate the model's performance during inference.

Specifically, for AR Diffusion, we carefully control the patch size to facilitate or hinder the model’s ability to learn feature relationships in a raster scan order. In Task 1, given a $32\times32$ input, we set the patch size to 16, ensuring the model learns sun-related features before shadow features, aligning with underlying dependencies. In contrast, for Task 2, we use a patch size of 8, causing different parts of the same square to appear in separate tokens, disrupting feature learning. By adjusting the patch size, we make Task 1 easier and Task 2 more challenging for AR Diffusion, allowing a direct comparison of its training and inference performance against DDPM under varying difficulty levels. Further details on synthetic data construction and model training are provided in Appendix~\ref{sec:app_more_training_details}. 


\begin{figure*}[]
\centering
    \hfill
    \subfigure[Training Data]{\label{fig:task2_tr}\includegraphics[width=0.24\textwidth]{figures/task2_tr.pdf}}
    \hfill
    \subfigure[Inference: AR Diffusion]{\label{fig:task2_ar}\includegraphics[width=0.24\textwidth]{figures/task2_ar.pdf}}
    \hfill
    \subfigure[Inference: DDPM]{\label{fig:task2_ddpm}\includegraphics[width=0.24\textwidth]{figures/task2_ddpm.pdf}}
    \hfill
    \subfigure[Training: Diffusion Loss]{\label{fig:task2_loss}\includegraphics[width=0.22\textwidth]{figures/task2_loss_distribution.pdf}}
    \hfill
\vspace{-0.15in}
\caption{\textbf{Comparison of AR Diffusion and DDPM Performance on Task 2.} \Cref{fig:task2_tr} demonstrates the validity of the evaluation method using the training data as a baseline.  
\Cref{fig:task2_ar} and \Cref{fig:task2_ddpm} illustrate the performance of AR Diffusion and DDPM during the inference phase, showing that AR Diffusion captures inter-feature dependencies less effectively, with a lower \( R^2 \).  
\Cref{fig:task2_loss} presents the difference in training loss between DDPM and AR Diffusion, denoted as \( \delta \). For most training steps, AR Diffusion's training loss is higher than that of DDPM, with \( \delta \leq 0 \).
.}
\vspace{-0.15in}
\label{fig:task_2_dis}
\end{figure*}

\paragraph{Results.}\Cref{fig:task_1_dis} and \cref{fig:task_2_dis} illustrate the performance of AR Diffusion and DDPM on the synthetic tasks, Task 1 and Task 2. Specifically, we evaluate both models in terms of their performance during inference and training.

\textit{Inference Phase.} Following \citet{han2025can}, we first extract geometric features from the training dataset and observe that for both Task 1 and Task 2 in \cref{fig:task1_tr} and \cref{fig:task2_tr}, the extracted geometric features (almost) perfectly satisfy the predefined feature dependencies, with an \( R^2 \) value (almost) equal to 1. The (almost) perfect estimation line further validates the effectiveness of the feature extraction method. Next, \cref{fig:task1_ar}, \cref{fig:task1_ddpm}, \cref{fig:task2_ar}, and \cref{fig:task2_ddpm} illustrate the generation quality of AR Diffusion and DDPM in both tasks, specifically whether the generated samples satisfy the predefined feature dependencies. We observe that for Task 1, AR Diffusion's generations better satisfy the predefined dependencies compared to DDPM, as indicated by larger \( R^2 \), whereas the opposite holds for Task 2. This demonstrates that when feature dependencies exist, given an appropriate patch partitioning, AR Diffusion’s learning paradigm can better capture these dependencies than DDPM.

Moreover, to further confirm that the key factor behind AR Diffusion's superior performance over DDPM in Task 1 stems from the advantage of AR Diffusion's next-token prediction paradigm in emphasizing inter-feature dependencies, \Cref{sec:Ablation: Parallel order} provides additional ablation experiments. Specifically, while keeping other factors unchanged, we modify only the learning order of AR Diffusion. Instead of using a raster scan order that aligns with the feature relationships—learning the sun region first and then the shadow region—we change it to a parallel order, where the sun and shadow regions are learned simultaneously, preventing AR Diffusion from correctly capturing inter-feature dependencies. We observe that the parallel order severely degrades AR Diffusion's generation quality, with \( R^2 \) dropping to $0.68$.

\textit{Training Phase.} \Cref{fig:task1_loss} and \Cref{fig:task2_loss} illustrate the loss differences between AR Diffusion and DDPM during training, where \( \delta := \mathcal{L}_{DDPM} - \mathcal{L}_{AR} \). Notably, the AR Diffusion loss incorporates the correction factor \( K \) derived in Theorem~\ref{thm:main_}. A sufficiently accurate correction factor can precisely characterize the training loss of all tokens in AR Diffusion, and a reasonable training loss should provide a sufficiently tight upper bound in Theorem~\ref{thm:main_} to faithfully reflect the model's generation quality during inference.  

We observe that for Task 1, where AR Diffusion outperforms DDPM in the inference phase, AR Diffusion loss is also lower than DDPM loss in approximately $76\%$ of training steps. Conversely, for Task 2, where AR Diffusion underperforms compared to DDPM in inference, its training loss is only lower than DDPM in only about $12\%$ of training steps. The consistency between AR Diffusion’s performance in the training and inference phases highlights the tightness of the upper bound in Theorem~\ref{thm:main_}. This observation also suggests a potential method for comparing the performance of AR Diffusion and DDPM—by comparing the corrected AR Diffusion training loss with DDPM training loss, we may be able to predict the model's performance during the inference phase.

\paragraph{Additional Experiments on Real-world Data.}
In addition, \cref{app:More Architectures and More Data} considers more real-world data. Specifically, we construct $2\times2$ composite images by concatenating MNIST digits, where the four digits satisfy predefined feature dependencies, such as forming an arithmetic sequence (e.g., $1, 2, 3, 4$) or all being even or odd numbers (e.g., $2, 2, 4, 4$). These additional experiments based on real data further support our analysis that AR learns the dependencies between non-independent features better than DDPM. Furthermore, the impacts of model architecture is also considered in \cref{app:More Architectures and More Data}, where we compare AR and DDPM using different backbones such as MLP and U-Net, and observe consistent conclusions with the experiments mentioned above.


% \Cref{fig:task_1_dis} and \cref{fig:task_2_dis} illustrate the experimental results, including the ratio distribution and the exponentially weighted moving average (EWMA) smoothed training loss \cite{hunter1986exponentially}, for AR Diffusion and DDPM on the two synthetic tasks. For Task 1, where the correlation between features (the side lengths of squares and rectangles) is easier for AR Diffusion to learn—thanks to its careful design ensuring that related objects are separated—AR Diffusion exhibits higher generation quality compared to DDPM. This is evident from the Ratio distribution being more concentrated around the target ratio of $1.5$ and the correspondingly lower training loss. In contrast, when inter-feature dependencies in Task 2 are difficult to learn through autoregressive modeling, AR Diffusion demonstrates disadvantages compared to DDPM. This is evident not only in the Ratio distribution being more uniform—while DDPM's distribution is more concentrated around the target ratio of $5$—but also in AR Diffusion's higher training loss.

% Notably, for Task 2, we also present the training loss of AR Diffusion before correction. This aligns with \cref{thm:main_}: the training losses before and after correction differ only by a factor of $K$, where $K$ is the number of patches (16 in Task A). The lower generation quality typically leads to higher training loss (as the dominant term), and our theoretically predicted factor of $K$ precisely explains why AR Diffusion exhibits higher training loss compared to DDPM. This experimentally validates the correctness of our theoretical result in \cref{thm:main_}.







==> 0_contents/050Experiments_v1.tex <==
\begin{figure*}
\centering
    \begin{minipage}{0.49\textwidth}
    \subfigure[Ratio Distribution]{\label{fig:task_1_dis}\includegraphics[width=0.49\textwidth]{figures/three_task1.pdf}}
        \subfigure[Smoothed Training Loss]{\label{fig:task_1_loss}\includegraphics[width=0.485\textwidth]{figures/square_rectangle_hard_200_patch16_ddpm_loss.pdf}}
        \vspace{-0.1in}
        \caption{Comparison between AR Diffusion (patch size = $16$) and DDPM on Task 1. AR Diffusion generates a higher density of samples with ratios closely aligned to the target value of $1.5$, while also achieving lower training losses.}
    \end{minipage}
    \begin{minipage}{0.49\textwidth}
        \centering
        \subfigure[Ratio Distribution]{\label{fig:task_2_dis}\includegraphics[width=0.49\textwidth]{figures/three_task2.pdf}}
        \subfigure[Smoothed Training Loss]{\label{fig:task_2_loss}\includegraphics[width=0.49\textwidth]{figures/gms_minmax_600_patch16_ddpm_loss.pdf}}
        \vspace{-0.1in}
        \caption{Comparison between AR Diffusion (patch size = $8$) and DDPM on Task 2. DDPM generates a higher density of samples with ratios closely aligned to the target value of $5$, while also achieving lower training losses.}
    \end{minipage}
% \vspace{-0.1in}
% \vspace{-0.15in}
\end{figure*}

\section{Experiment}
\label{sec:exp}
In this section, we demonstrate the advantages of AR Diffusion over DDPM in two synthetic experiments, where the image data contains both explicit and subtle feature dependencies, respectively.

\paragraph{Synthetic Tasks.}Specifically, we consider the following synthetic tasks in \cref{fig:task_vis}: (1) Task 1: Contains a square and a rectangle, where the side length $l_1$ of the square in the upper half and the side length $l_2$ of the rectangle in the lower half satisfy the constraint $l_2 = 1.5l_1$; (2) Task 2: Contains two rectangles, where the side length $l_1$ of the square in the upper half and the side length $l_2$ of the rectangle in the lower half satisfy the constraint $l_2 = 5l_1$.  

To construct the synthetic data with explicit and subtle dependencies, we carefully design the Patch Size for sequential learning of the two features.
Taking Task 1 as an example, for $32 \times 32$ image data, \cref{fig:task1} sets the patch size to 16, ensuring the square always appears in the first patch while the rectangle appears in the fourth patch, which shows an explicit patch dependence since $l_2 = 1.5l_1$.
In contrast, as shown in \cref{fig:task2}, when the patch size is set to $8$ for $32 \times 32$ image data, both rectangles may appear within the same patch (e.g., patch $9$), which makes the patch dependence subtle, and poses challenges for learning inter-feature relationships.

\begin{figure}[]
\centering
    \hfill
    \subfigure[Task 1]{\label{fig:task1}\includegraphics[width=0.2\textwidth]{figures/task1.pdf}}
    \hfill
    \subfigure[Task 2]{\label{fig:task2}\includegraphics[width=0.2\textwidth]{figures/task2.pdf}}
    \hfill
\vspace{-0.1in}
\caption{Visualization of Task 1 and Task 2. Through careful design, Task 1 ensures that dependent objects are placed in different patches, making it easier for the autoregressive approach to learn feature correlations. Task 2 is more complex with dependent features located within the same patch, which poses challenges for learning inter-feature relationships.}
\vspace{-0.15in}
\label{fig:task_vis}
\end{figure}
\paragraph{Setup and Evaluation.} 
For each task, we synthesize 2000 samples and use them to train both AR Diffusion and DDPM. For AR Diffusion, we adopt a simplified version without VAE, training directly in pixel space to preserve inter-feature relationships. To ensure a fair comparison, AR Diffusion and DDPM are configured with consistent total model parameters and training epochs. We use U-Net as the denoising neural network for DDPM and MLP for AR Diffusion, with a learning rate of $3e-4$ and approximately $23M$ model parameters. Training is conducted on a single NVIDIA A800 GPU for $200$ epochs (Task 1) and $600$ epochs (Task 2), respectively.
For the generated images, we can directly obtain image masks using predefined colors (e.g., red or blue for the square and rectangle in Task 1) during image generation. Using these masks, we can directly extract the variables of interest, such as the square's side length $l_1$ and the rectangle's side length $l_2$, and calculate their ratio $R = \frac{l_2}{l_1}$. For Task 1, the target ratio is $R = 1.5$, while for Task 2, the target ratio is $R = 5$.

\paragraph{Results.}
\Cref{fig:task_1_dis} and \cref{fig:task_2_dis} illustrate the experimental results, including the ratio distribution and the exponentially weighted moving average (EWMA) smoothed training loss \cite{hunter1986exponentially}, for AR Diffusion and DDPM on the two synthetic tasks. For Task 1, where the correlation between features (the side lengths of squares and rectangles) is easier for AR Diffusion to learn—thanks to its careful design ensuring that related objects are separated—AR Diffusion exhibits higher generation quality compared to DDPM. This is evident from the Ratio distribution being more concentrated around the target ratio of $1.5$ and the correspondingly lower training loss. In contrast, when inter-feature dependencies in Task 2 are difficult to learn through autoregressive modeling, AR Diffusion demonstrates disadvantages compared to DDPM. This is evident not only in the Ratio distribution being more uniform—while DDPM's distribution is more concentrated around the target ratio of $5$—but also in AR Diffusion's higher training loss.

Notably, for Task 2, we also present the training loss of AR Diffusion before correction. This aligns with \cref{thm:main_}: the training losses before and after correction differ only by a factor of $K$, where $K$ is the number of patches (16 in Task A). The lower generation quality typically leads to higher training loss (as the dominant term), and our theoretically predicted factor of $K$ precisely explains why AR Diffusion exhibits higher training loss compared to DDPM. This experimentally validates the correctness of our theoretical result in \cref{thm:main_}.







==> 0_contents/060conclusion.tex <==
\section{Conclusion}
In conclusion, this work presents a novel theoretical and practical exploration into the strengths of AR diffusion models compared to standard diffusion approaches. 
AR diffusion leverages a stage-wise auto-regressive structure that more effectively captures conditional dependencies in high-dimensional data. 
The key findings establish that AR diffusion converges in terms of the KL divergence for each conditional distribution, whereas vanilla diffusion models can fail to preserve these conditional distributions even when the joint distribution converges. 
Furthermore, AR diffusion retains near-minimal assumptions on the data distribution and score smoothness.

For future work, in addition to SDE-based inference, various ODE-based inference methods have been extensively studied in typical DDPM \citep{li2024towards,chen2024probability,li2024sharp}.
It will be intriguing to investigate whether the Fokker--Planck equivalence can be adapted to auto-regressive settings and whether ODE-based inference can retain its convergence.
Besides, the theoretical properties of some high-order ODE or SDE-based inference algorithms \citep{wu2024stochastic,lu2022dpm} remain unknown.
Moreover, various works \citep{han2024neural, chen2024overview} have started to investigate the optimization and generalization properties. 

==> 0_contents/backup.tex <==
\textcolor{red}{\hrule}




Besides, we denote the underlying distribution of $\rvy_0$ is $p_{*,k|\vx_{[1:k-1]}}(\cdot|\vx_{[1:k-1]})$ and the underlying distribution of $\rvy_t$ as $q_t$, respectively.
To simplify the notations, we will not distinguish different $\vtheta$s strictly and only use $\vtheta$ to present the trainable parameters we are concerned with.
By supposing 

the inference process of AR diffusion shown in \citet{li2024autoregressive} can be simplified as Alg.~\ref{alg:ard_outer}.

%----------- Jan 19

\textcolor{red}{\hrule}
    
    
    \paragraph{Control the first term in Eq.~\ref{ineq:causal_discrete_error}.}
    We suppose $c_{y}(t) = \left(e^{-2t}\sigma^2 +1 - e^{-2t}\right)^{-1}$ and have
    \begin{equation*}
        c_y^\prime(t) = \frac{2\left(\sigma^2 - 1\right)e^{2t}}{\left(e^{2t} + \sigma^2 - 1\right)^2}.
    \end{equation*}
    When $\sigma\ge 1$, it has
    \begin{equation}
        \label{ineq:c_y_upb_1}
        |c_y^\prime(t)| \le \frac{2(\sigma^2 -1)e^{2t}}{e^{4t}} = 2(\sigma^2 -1)e^{-2t}\le 2(\sigma^2 -1).
    \end{equation}
    When $1\ge \sigma^2>0$ and 
    \begin{equation*}
        e^{2t} + \sigma^2 -1 \ge \frac{e^{2t}}{2}\quad \Leftrightarrow\quad t\ge \frac{\ln 2(1-\sigma^2)}{2},
    \end{equation*}
    it has
    \begin{equation}
        \label{ineq:c_y_upb_2}
        |c_y^\prime(t)| \le 2(1-\sigma^2)e^{2t}\cdot 4e^{-4t} = 8(1-\sigma^2)\cdot e^{-2t}\le  8(1-\sigma^2).
    \end{equation}
    Otherwise, i.e., when $1\ge \sigma^2>0$ and $t\le \ln 2(1-\sigma^2)/2$, it has
    \begin{equation}
        \label{ineq:c_y_upb_3}
        |c_y^\prime(t)| \le \frac{4(\sigma^2 -1)^2}{\sigma^4} \le 4(1-\sigma^2)\sigma^{-4}
    \end{equation}
    Combining Eq.~\ref{ineq:c_y_upb_1}, Eq.~\ref{ineq:c_y_upb_2} and Eq.~\ref{ineq:c_y_upb_3}, we have
    \begin{equation*}
        |c_y^\prime(t)|\le C_1(\sigma)\coloneqq 8\left|\sigma^2-1\right|\cdot \max\left\{1, \sigma^{-4}\right\}.
    \end{equation*}
    Then, Term 1 of Eq.~\ref{eq:causal_score_diff} can be upper bounded by
    \begin{equation*}
        \begin{aligned}
            \left|\text{Term 1}\right| = \left|c_y(T-t) - c_y(T-r\eta)\right|  = \left|\int_{T-r\eta}^{T-t} c_y^\prime(\tau) \der \tau\right| \le (t-r\eta)\cdot C_1(\sigma).
        \end{aligned}
    \end{equation*}
    We use a similar technique, we suppose $c_x(t) = e^{-t}/(e^{-2t}\sigma^2 + 1 - e^{-2t})$ and have
    \begin{equation*}
        |c_x^\prime(t)| = \frac{e^{2t}}{\left(e^{2t}+\sigma^2 - 1\right)^2}.
    \end{equation*}
    When $\sigma\ge 1$, it has
    \begin{equation}
        \label{ineq:c_x_upb_1}
        |c_x^\prime(t)| \le e^{-2t}\le 1.
    \end{equation}
    When $1\ge \sigma^2>0$ and 
    \begin{equation*}
        e^{2t} + \sigma^2 -1 \ge \frac{e^{2t}}{2}\quad \Leftrightarrow\quad t\ge \frac{\ln 2(1-\sigma^2)}{2},
    \end{equation*}
    it has
    \begin{equation}
        \label{ineq:c_x_upb_2}
        |c_x^\prime(t)| \le e^{2t} \cdot 4e^{-4t} \le 4.
    \end{equation}
    Otherwise, i.e., when $1\ge \sigma^2>0$ and $t\le \ln 2(1-\sigma^2)/2$, it has
    \begin{equation}
        \label{ineq:c_x_upb_3}
        |c_x^\prime(t)| \le 2(1-\sigma^2)\cdot \sigma^{-4}.
    \end{equation}
    Combining Eq.~\ref{ineq:c_x_upb_1}, Eq.~\ref{ineq:c_x_upb_2} and Eq.~\ref{ineq:c_x_upb_3}, we have
    \begin{equation*}
        |c_x^\prime(t)|\le C_2(\sigma)\coloneqq 4\max\left\{1, \sigma^{-4}\right\}.
    \end{equation*}
    Then, Term 2 of Eq.~\ref{eq:causal_score_diff} can be upper bounded by
    \begin{equation*}
        \begin{aligned}
            \left|\text{Term 2}\right| = \left|c_x(T-t) - c_x(T-r\eta)\right|  = \left|\int_{T-r\eta}^{T-t} c_y^\prime(\tau) \der \tau\right| \le (t-r\eta)\cdot C_2(\sigma).
        \end{aligned}
    \end{equation*}
    Under these conditions, Eq.~\ref{eq:causal_score_diff} can be rewritten as
    \begin{equation*}
        \left\|\grad\ln q_{T-r\eta}(\vy) - \grad\ln q_{T-t}(\vy)\right\|^2 \le 2 (t-r\eta)^2\cdot \left( C_1^2(\sigma)\|\vy\|^2 + C_2^2(\sigma)\|\vx_1\|^2\right),
    \end{equation*}
    which implies
    \begin{equation}
        \label{ineq:casual_term1_upb}
        \begin{aligned}
        &\E_{\tilde{\rvy}_{[0:T]}}\left[\left\|\grad\ln q_{T-r\eta}(\tilde{\rvy}_{r\eta}) - \grad\ln q_{T-t}(\tilde{\rvy}_{r\eta})\right\|^2\right]\le 2(t-r\eta)^2\cdot \left(C_1^2(\sigma)\E[\|\tilde{\rvy}_{r\eta}\|^2]+ C_2^2(\sigma)\|\vx_1\|^2\right)  \\
        & \le 2(t-r\eta)^2\cdot \left(C_1^2(\sigma)\E[\|\rvy_{T - r\eta}\|^2]+ C_2^2(\sigma)\|\vx_1\|^2\right) \le 2(t-r\eta)^2 \cdot \left(C_1^2(\sigma)\E[\|\rvy_0\|^2] + C_1^2(\sigma)d + C_2^2(\sigma)\|\vx_1\|^2\right)\\
        & = 2(t-r\eta)^2\cdot \left(C_1^2(\sigma)\E_{\rvx_2\sim p_{*,2|1}(\cdot|\vx_1)}[\|\rvx_2\|^2]+C_1^2(\sigma)d + C_2^2(\sigma)\|\vx_1\|^2\right).
        \end{aligned}
    \end{equation}
    It should be noted that the third inequality follows from the fact
    \begin{equation*}
        \rvy_t = e^{-t}\cdot \rvy_0 + \sqrt{1-e^{-2t}}\xi \quad \Leftrightarrow\quad \E[\|\rvy_t\|^2]  = e^{-2t}\E[\|\rvy_0\|^2] + (1-e^{-2t})\E[\|\xi\|^2]\le \E[\|\rvy_0\|^2]+d.
    \end{equation*}
    \paragraph{Control the second term in Eq.~\ref{ineq:causal_discrete_error}.} According to the closed form of $q_t$ shown in Eq.~\ref{ineq:causal_q_t_close_form}, we have
    \begin{equation*}
        \grad^2 \ln q_{T-t}(\vy) = 
    \end{equation*}


%--------------- RTK bound

\begin{lemma}
    \label{lem:kl_to_drift_diff}
    TBC
\end{lemma}
\begin{proof}
    According to the update rule of particles shown in Eq.~\ref{step:inner_sampler} of Alg.~\ref{alg:ard_inner}, the practical transition kernel $q^\gets_{t_{r+1}|t_r}(\vy^\prime|\vy)$ can be written as
    \begin{equation*}
        q^\gets_{t_{r+1}|t_r}(\vy^\prime|\vy)\propto \exp\left(-\frac{\left\|\vy^\prime - \left(e^{\eta_r}\vy + (e^{\eta_r}-1)\cdot 2\vs_{\vtheta}(\vy|t_R-t_r,\vz\right)\right\|^2}{2\cdot (e^{2\eta_r - 1})}\right)
    \end{equation*}
    which is a Gaussian-type distribution having a linear score
    \begin{equation}
        \label{eq:score_prac_rtk_fin}
        \begin{aligned}
            &\grad_{\vy^\prime}q^\gets_{t_{r+1}|t_r}(\vy^\prime|\vy) = -\frac{\vy^\prime - \left(e^{\eta_r}\cdot \vy + 2(e^{\eta_r}-1)\cdot \vs_\vtheta(\vy|t_R-t_r, \vz)\right)}{e^{2\eta_r} - 1}\\
            & = \frac{2(e^{\eta_r}-1)}{e^{2\eta_r}-1}\cdot \vs_\vtheta(\vy|T-t_r, \vz) + \frac{\vy}{e^{\eta_r} - e^{-\eta_r}} - \frac{\vy^\prime}{e^{2\eta_r}-1}
        \end{aligned}
    \end{equation}
    and strong log-concavity, i.e.,
    \begin{equation*}
        - \grad_{\vy^\prime}^2\ln q^\gets_{t_{r+1}|t_r}(\vy^\prime|\vy) = \left(e^{2\eta_r} - 1\right)^{-1}.
    \end{equation*}
    Note that the last equation of Eq.~\ref{eq:score_prac_rtk_fin} follows from $t_R = T$ in the definition Eq.~\ref{def:time_eta_seq}.
    Then, according to Lemma~\ref{lem:strongly_lsi}, we have
    \begin{equation}
        \label{ineq:kl_upb_fi}
        \KL{\tilde{q}_{t_{r+1}|t_r}(\cdot|\vy)}{q^\gets_{t_{r+1}|t_r}(\cdot|\vy)} \le \frac{e^{2\eta_r}-1}{2}\cdot \int \tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy)\cdot \left\|\grad\ln \frac{\tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy)}{q^\gets_{t_{r+1}|t_r}(\vy^\prime|\vy)}\right\|^2 \der \vy^\prime.
    \end{equation}
    Considering that
    \begin{equation}
        \label{eq:score_ideal_rtk_p1}
        \begin{aligned}
            &\tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy)\cdot \tilde{q}_{t_r}(\vy) = q_{T-t_{r+1}|T-t_r}(\vy^\prime|\vy)\cdot q_{T-t_r}(\vy) = q_{T-t_r|T-t_{r+1}}(\vy|\vy^\prime)\cdot q_{T-t_{r+1}}(\vy^\prime)\\
            & \Leftrightarrow \grad_{\vy^\prime}\ln \tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy) = \grad_{\vy^\prime}\ln q_{T-t_{r+1}}(\vy^\prime) + \grad_{\vy^\prime}\ln q_{T-t_r|T-t_{r+1}}(\vy|\vy^\prime).
        \end{aligned}
    \end{equation}
    Since the forward process of $\rvy_t\sim q_t$ follows from the OU process, the forward transition kernel $q_{T-t_r|T-t_{r+1}}(\vy|\vy^\prime)$ satisfies
    \begin{equation}
        \label{eq:score_ideal_rtk_p2}
        \begin{aligned}
            & q_{T-t_r|T-t_{r+1}}(\vy|\vy^\prime) \propto \exp\left(-\frac{\left\|\vy - e^{-(t_{r+1}-t_r)}\cdot \vy^\prime\right\|^2}{2\cdot (1-e^{-2(t_{r+1}-t_r)})}\right) = \exp\left(-\frac{\left\|\vy - e^{-\eta_r}\cdot \vy^\prime\right\|^2}{2(1-e^{-2\eta_r})}\right)\\
            & \Leftrightarrow\ \grad_{\vy^\prime}\ln q_{T-t_r|T-t_{r+1}}(\vy|\vy^\prime) =  \frac{\vy - e^{-\eta_r}\cdot\vy^\prime}{1-e^{-2\eta_r}}\cdot e^{-\eta_r} = \frac{\vy}{e^{\eta_r} - e^{-\eta_r}}  - \frac{\vy^\prime}{e^{2\eta_r} - 1}.
        \end{aligned}
    \end{equation}
    Plugging Eq.~\ref{eq:score_ideal_rtk_p2} into Eq.~\ref{eq:score_ideal_rtk_p1}, we have
    \begin{equation}
        \label{eq:score_ideal_rtk_fin}
        \grad_{\vy^\prime}\ln \tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy) = \grad_{\vy^\prime}\ln q_{T-t_{r+1}}(\vy^\prime) + \frac{\vy}{e^{\eta_r} - e^{-\eta_r}}  - \frac{\vy^\prime}{e^{2\eta_r} - 1}.
    \end{equation}
    Plugging Eq.~\ref{eq:score_ideal_rtk_fin} and Eq.~\ref{eq:score_prac_rtk_fin} into Eq.~\ref{ineq:kl_upb_fi}, we have
    \begin{equation*}
        \begin{aligned}
            &\KL{\tilde{q}_{t_{r+1}|t_r}(\cdot|\vy)}{q^\gets_{t_{r+1}|t_r}(\cdot|\vy)}\le \frac{e^{2\eta_r}-1}{2}\cdot \int \tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy)\cdot \left\|\frac{2(e^{\eta_r}-1)}{e^{2\eta_r}-1}\cdot \vs_\vtheta(\vy|T-t_r, \vz) - \grad_{\vy^\prime}\ln q_{T-t_{r+1}}(\vy^\prime) \right\|^2 \der \vy^\prime\\
            & \le (e^{2\eta_r}-1)\cdot \left(\frac{2(e^{\eta_r}-1)}{e^{2\eta_r}-1}\right)^2\cdot \int \tilde{q}_{t_{r+1}|t_r}(\vy^\prime|\vy)\cdot \left\|\vs_\vtheta(\vy|T-t_r, \vz) - \grad_{\vy^\prime}\ln q_{T-t_{r+1}}(\vy^\prime)\right\|^2 \der \vy^\prime\\
            &\quad + (e^{2\eta_r}-1)\cdot \left(\frac{2(e^{\eta_r}-1)}{e^{2\eta_r}-1} - 1\right)^2 \cdot 
        \end{aligned}
    \end{equation*}
\end{proof}

since the practical transition $q^\gets_{t_{r+1}|t_r}(\cdot|\tilde{\rvy})$ is Gaussian-type due to Eq.~\ref{sde:prac_condi_reverse}, and the reverse transition $\tilde{q}_{t_{r+1}|t_r}(\cdot|\tilde{\rvy})$ has analytic form provided  in \citet{huang2024reverse}, respectively,
Lemma~\ref{}


% Jan 22---------------------------------

Under the assumptions stated in Section~\ref{sec:pre}, this section shows that the AR diffusion model attains nearly the same gradient complexity as standard diffusion, differing only by an additional factor of $K$ when achieving TV or KL convergence.
To reach this conclusion, we methodically unveil the theoretical properties of AR diffusion models by answering three principal questions on both the training and inference stages:
\begin{enumerate}
    \item How does the training loss in Eq.~\ref{eq:obj_ard_p} connect to the commonly used score estimation error in existing diffusion studies?
    \item What is the entire forward and reverse process of AR diffusions corresponding to the ground-truth scores?
    \item How can we require the generated sample to be close to the data by managing the score estimation and discretization errors in tokens' generation and concatenation?
\end{enumerate}


\textcolor{red}{\hrule}

Following \citet{li2024autoregressive}, we briefly revisit autoregressive diffusion generation, summarized by Alg.~\ref{alg:ard_outer}:
specifically, when generating token $(k+1)$, it should be conditioned on all previously generated tokens, $\vx_{[1:k]}$ or their representations, i.e., $\vz$ in Eq.~\ref{eq:conditioning_gene}.
Under this condition, we suppose the generated $\rvx_{k+1}^\gets$ follows a distribution $q_{0}(\cdot|\vx_{[1:k]})$ which can be transformed to the standard Gaussian with the following SDE, i.e.,

Then, sampling $\rvx^\gets_{k+1}$ can be regarded as reversing the SDE.~\ref{sde:ideal_condi_forward} by simulating

which satisfies $\tilde{q}_t = q_{T-t}$.
Therefore, Alg.~\ref{alg:ard_outer} invokes Alg.~\ref{alg:ard_inner} to solve


which estimates Eq.~\ref{sde:ideal_condi_reverse} and has an analytic solution Eq.~\ref{sde:prac_condi_reverse} due to the exponential integrator.



As described in Eq.~\ref{def:time_eta_seq}, 

To guarantee the KL convergence for arbitrary small error tolerance, i.e., $\epsilon$, a sufficient condition is to require
\begin{equation*}
    \small
    \begin{aligned}
        &\KL{p_{*,1}}{p^\gets_{*,1}}\le \epsilon^2/K \quad \text{and}\\
        & \E
        \left[\KL{p_{*,k+1|[1:k]}(\cdot|\rvx_{[1:k]})}{p^\gets_{*,k+1|[1:k]}(\cdot|\rvx_{[1:k]})}\right]\le \epsilon^2/K
    \end{aligned}
\end{equation*}
where $p^\gets_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})$ is equivalent to the distribution $q^\gets_T$ of the output particle of Alg.~\ref{alg:ard_inner} for any given tokens $\vx_{[1:k]}$ or their representations $\vz$.
Then, the KL divergence between $q^\gets_T$ and the conditional data distribution, i.e., $\tilde{q}_T = p_{*,k+1|[1:k]}(\cdot|\vx_{[1:k]})$ will be


In our work, we main focus on the sampling process of the AR diffusion model. To approach this, we assume that the ground truth score can be well learned with up to small estimation errors. The assumption on Eq.~\ref{eq:ard_global_loss} is made as follows:


% ------------- Jan. 30:

According to the definition, AR is intuitively well-suited for capturing conditional dependencies among features, while its widespread use in practical applications primarily stems from its promising scalability when implemented with Transformer-based neural networks.
In addition to the well-known applications in natural language processing~\citep{radford2018improving,radford2019language,brown2020language}, image generation~\citep{tian2024visual,yu2024randomized}, and text-to-speech synthesis~\citep{arik2017deep,ping2018clarinet}, a new paradigm adopts AR in denoising diffusion generative models, attracting significant attention in recent years. Initially introduced for image generation~\citep{li2024autoregressive}, AR diffusion has been applied in diverse real-world scenarios, including text-to-speech synthesis~\citep{meng2024autoregressive} and video generation~\citep{liu2024mardini}.
Moreover, such empirical success motivates us to theoretically investigate the fundamental properties of AR, especially for its generation quality and efficiency.

==> temp_images/dimension_reduction_forward.tex <==
\begin{tikzpicture}
% Initialization data distribution
\node at (-0.5, -7.5) {\small $\rvx_0\sim u_0$};
\node at (-0.5, -10) {\small
    $\left[\begin{aligned}
        &\rx_{0,1}\\
        &\rx_{0,2}\\
        &\ldots\\
        &\rx_{0,d^\prime}\\
        &\rx_{0,d^\prime+1}\\
        &\ldots\\
        &\rx_{0,d}
    \end{aligned}\right]$
};
\draw[-latex] (0.5,-10)--(1.5,-10);
\node at (1, -9.8) {\small $\mQ^\top$};

% Starting distribution at t=0
\node at (2.5, -7.5) {\small $(\rvx^\to_0, \rvy^\to_0)\sim u^\to_0$};
\node at (2.5, -10) {\small
    $\left[\begin{aligned}
        &\textcolor{red}{\rx^\to_{0,1}}\\
        &\textcolor{red}{\rx^\to_{0,2}}\\
        &\textcolor{red}{\ldots}\\
        &\textcolor{red}{\rx^\to_{0,d^\prime}}\\
        &\textcolor{blue}{\ry^\to_{0,1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\to_{0,d-d^\prime}}
    \end{aligned}\right]$
};

\draw[-latex] (3.5,-9)--(4,-9);
\draw[-latex] (3.5,-11)--(4,-11);
\node at (5.5, -9) {\small
    $\left[\begin{aligned}
        &\textcolor{red}{\rx^\to_{0,1}}\\
        &\textcolor{red}{\rx^\to_{0,2}}\\
        &\textcolor{red}{\ldots}\\
        &\textcolor{red}{\rx^\to_{0,d^\prime}}\\
    \end{aligned}\right]\sim p_0^\to(\cdot|\rvy_0)$
};

\node at (5.3, -11) {\small
    $\left[\begin{aligned}
        &\textcolor{blue}{\ry^\to_{0,1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\to_{0,d-d^\prime}}
    \end{aligned}\right]\sim q_0^\to$
};

%Towards K_1
\node at (7.5, -8.8) {\small $\mathrm{FTK}_1$};
\draw[-latex] (7,-9)--(8,-9);
\node at (9.5, -8.8) {\small $\rvx^\to_{K_1}\sim p^\to_{K_1}(\cdot|\rvy_0)$};
\node at (9.9, -9.2) {\small $p^\to_{K_1}(\cdot|\rvy_0) \approx \mathcal{N}\left(\vzero, \mI_{d^\prime}\right)$};

\node at (7.5, -10.8) {\small Fixed};
\draw[-latex] (6.5,-11)--(8.5,-11);
\node at (9.5, -11) {\small
    $\left[\begin{aligned}
        &\textcolor{blue}{\ry^\to_{K_1,k+1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\to_{K_1,d}}
    \end{aligned}\right]$
};

\draw [decorate,decoration={brace,amplitude=5pt, mirror}] (5,-11.8) -- (9.5,-11.8);
\node at (7.25, -12.3) {\small Stage 1};

%Toward K_2
\draw[-latex] (10.5,-11)--(12.5,-11);
\node at (11.5, -10.8) {\small $\mathrm{FTK}_2$};
\node at (14, -10.8) {\small $\rvy^\to_{K_1+K_2}\sim q^\to_{K_1+K_2}$};
\node at (14.2, -11.2) {\small $q^\to_{K_1+K_2}\approx \mathcal{N}\left(\vzero, \mI_{d-d^\prime}\right)$};
\draw [decorate,decoration={brace,amplitude=5pt, mirror}] (9.5,-11.8) -- (14,-11.8);
\node at (11.75, -12.3) {\small Stage 2};




% Division

\node at (6, -13.5) {\textbf{Forward Process}};
\draw [line width=0.25mm] (-2,-14) -- (14,-14);
\node at (6, -14.5) {\textbf{Reverse Process}};

% Reverse Process


\node at (-0.5, -15.5) {\small $\tilde{\rvx}_0\sim \tilde{u}_0$};
\node at (-0.5, -18) {\small
    $\left[\begin{aligned}
        &\tilde{\rx}_{0,1}\\
        &\tilde{\rx}_{0,2}\\
        &\ldots\\
        &\tilde{\rx}_{0,d^\prime}\\
        &\tilde{\rx}_{0,d^\prime+1}\\
        &\ldots\\
        &\tilde{\rx}_{0,d}
    \end{aligned}\right]$
};
\draw[-latex] (1.5,-18)--(0.5,-18);
\node at (1, -17.8) {\small $\mQ$};

% Starting distribution at t=0
\node at (2.5, -15.5) {\small $(\rvx^\gets_0, \rvy^\gets_0)\sim u^\gets_0$};
\node at (2.5, -18) {\small
    $\left[\begin{aligned}
        &\textcolor{red}{\rx^\gets_{0,1}}\\
        &\textcolor{red}{\rx^\gets_{0,2}}\\
        &\textcolor{red}{\ldots}\\
        &\textcolor{red}{\rx^\gets_{0,d^\prime}}\\
        &\textcolor{blue}{\ry^\gets_{0,1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\gets_{0,d-d^\prime}}
    \end{aligned}\right]$
};

\draw[-latex] (4,-17)--(3.5,-17);
\draw[-latex] (4,-19)--(3.5,-19);
\node at (5.5, -17) {\small
    $\left[\begin{aligned}
        &\textcolor{red}{\rx^\gets_{0,1}}\\
        &\textcolor{red}{\rx^\gets_{0,2}}\\
        &\textcolor{red}{\ldots}\\
        &\textcolor{red}{\rx^\gets_{0,d^\prime}}\\
    \end{aligned}\right]\sim p_0^\gets(\cdot|\rvy_0)$
};

\node at (5.3, -19) {\small
    $\left[\begin{aligned}
        &\textcolor{blue}{\ry^\gets_{0,1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\gets_{0,d-d^\prime}}
    \end{aligned}\right]\sim q_0^\gets$
};

%Towards K_1
\node at (7.5, -16.8) {\small $\mathrm{RTK}_1$};
\draw[-latex] (8,-17)--(7,-17);
\node at (9.5, -16.8) {\small $\rvx^\gets_{K_1}\sim p^\gets_{K_1}(\cdot|\rvy_0)$};
\node at (9.9, -17.2) {\small $p^\gets_{K_1}(\cdot|\rvy_0) = \mathcal{N}\left(\vzero, \mI_{d^\prime}\right)$};

\node at (7.5, -18.8) {\small Fixed};
\draw[-latex] (8.5,-19)--(6.5,-19);
\node at (9.5, -19) {\small
    $\left[\begin{aligned}
        &\textcolor{blue}{\ry^\gets_{K_1,k+1}}\\
        &\textcolor{blue}{\ldots}\\
        &\textcolor{blue}{\ry^\gets_{K_1,d}}
    \end{aligned}\right]$
};

\draw [decorate,decoration={brace,amplitude=5pt, mirror}] (5,-19.8) -- (9.5,-19.8);
\node at (7.25, -20.3) {\small Reverse Stage 1};

%Toward K_2
\draw[-latex] (12.5,-19)--(10.5,-19);
\node at (11.5, -18.8) {\small $\mathrm{RTK}_2$};
\node at (14, -18.8) {\small $\rvy^\gets_{K_1+K_2}\sim q^\gets_{K_1+K_2}$};
\node at (14.2, -19.2) {\small $q^\gets_{K_1+K_2}= \mathcal{N}\left(\vzero, \mI_{d-d^\prime}\right)$};
\draw [decorate,decoration={brace,amplitude=5pt, mirror}] (9.5,-19.8) -- (14,-19.8);
\node at (11.75, -20.3) {\small Reverse Stage 2};



\end{tikzpicture}
